A study of muon-electron elastic scattering in a test beam

In 2018, a test run with muons in the North Area at CERN was performed, running parasitically downstream of the COMPASS spectrometer. The aim of the test was to investigate the elastic interactions of muons on atomic electrons, in an experimental configuration similar to the one proposed by the project MUonE, which plans to perform a very precise measurement of the differential cross-section of the elastic interactions. COMPASS was taking data with a 190 GeV pion beam, stopped in a tungsten beam dump: the muons from these pions decays passed through a setup including a graphite target followed by 10 planes of Si tracker and a BGO crystal electromagnetic calorimeter placed at the end of the tracker. The elastic scattering events were analysed, and compared to expectations from MonteCarlo simulation.

==> issuenr.tex <==
% if you write for a special issue this may be useful
\proceeding{N$^{\text{th}}$ Workshop on X\\
  when\\
  where}

==> setup_old_calo_backup.tex <==
\paragraph{The electromagnetic calorimeter}
In the data set analysed in this paper, the calorimeter was a compact array of
 $3 \times 3$ PbWO$_4$ crystals, with a volume of 
${2.1 \times 2.1 \times 23~\mbox{cm}^3}$ each, and readout
% of the output electron energy. 
by photodetectors Hamamatsu H6780-03 PMTs [97], whose sensitivity peak 
wavelength perfectly matches those of the PbWO4 emission peak.
The crystals were spare pieces of the CMS endcap calorimeter %\cite{ref95 tesi mattia}, 
arranged as shown in fig.\ref{STEFI_calo} 
%The CMS PbWO4 crystals have been extensively tested \cite{ref96 test mattia}.


\begin{figure}[htbp]
\centering % \begin{center}/\end{center} takes some additional vertical space
\includegraphics[width=.5\textwidth]{calo_STEFI.pdf}
\label{STEFI_calo}
\caption{ Scheme of STEFI \cite{Soldani_Master2019}.}
\end{figure}

Each crystal is contained in a custom aluminum box with a plastic plug for the 
coupling to the photodetector; the whole matrix is held together by a Bosch 
structure and is contained in a $\sim$ 50 cm long aluminum box 
%(photo in figure 2.24 left). 
It is trapezoidal, with a front section of 2.86 $\times$ 2.86 cm2, a rear 
section of $2.96 \times 2.96$ cm$^2$ and a length of 22 cm, which corresponds to
 $\sim$ 24.7 X$_0$. 
It is wrapped in a Tyvek sheet to increase the light yield. 
%\cite{ref 95 di mattia}[95].

Figure \ref{STEFI_calo} clearly shows that there is a few-mm gap between the 
different channels active areas due to the mechanical structure: these dead 
regions inside the active volume cause an energy loss and thus negatively  
affect the detector energy resolution. 

The results of the performance of STEFI are given in figures 
\ref{linearity_calo} and 
\ref{resolution_calo}.

The energy resolution turns out to $\sigma(E)= \sqrt (a/\sqrt(E))^2 + c^2$
with a=19.7$\%$ and c=15.1$\%$
\textcolor{red} {WARNING!!! check if STEFI or GENNI!!!!}

\textcolor{red}{Also describe saturation.....}

\begin{figure}[htbp]
\centering % \begin{center}/\end{center} takes some additional vertical space
\includegraphics[width=.5\textwidth]{calo_linearity.pdf}
\label{linearity_calo}
\caption{ Calorimeter linearity \cite{Soldani_Master2019}.}
\end{figure}

\begin{figure}[htbp]
\centering % \begin{center}/\end{center} takes some additional vertical space
\includegraphics[width=.5\textwidth]{calo_en-res.pdf}
\label{resolution_calo}
\caption{ Energy resolution \cite{Soldani_Master2019}.}
\end{figure}

Details of this calorimeter and on its characterization can be found in \cite{Soldani_Master2019}.

The trasverse size of the calorimeter covered an acceptance of about \textcolor{red}{(chiedere a Mattia distanza dalla target)}

==> testsec.tex <==
\section{Section 1}

THIS IS JUST A TEST SECTION \cite{test2}. SEE ALSO \cite{test1}.
